R-PRM: Reasoning-Driven Process Reward Modeling

Large language models (LLMs) inevitably make mistakes when performing step-by-step mathematical reasoning. Process Reward Models (PRMs) have emerged as a promising solution by evaluating each reasoning step. However, existing PRMs typically output evaluation scores directly, limiting both learning efficiency and evaluation accuracy, which is further exacerbated by the scarcity of annotated data. To address these issues, we propose Reasoning-Driven Process Reward Modeling (R-PRM). First, we leverage stronger LLMs to generate seed data from limited annotations, effectively bootstrapping our model's reasoning capabilities and enabling comprehensive step-by-step evaluation. Second, we further enhance performance through preference optimization, without requiring additional annotated data. Third, we introduce inference-time scaling to fully harness the model's reasoning potential. Extensive experiments demonstrate R-PRM's effectiveness: on ProcessBench and PRMBench, it surpasses strong baselines by 11.9 and 8.5 points in F1 scores, respectively. When applied to guide mathematical reasoning, R-PRM achieves consistent accuracy improvements of over 8.5 points across six challenging datasets. Further analysis reveals that R-PRM exhibits more comprehensive evaluation and stronger generalization capabilities, thereby highlighting its significant potential.

==> latex/fig/case-study-2.tex <==
\begin{figure*}[t]
% \setlength\extrarowheight{3pt}
\vspace{-0.2cm}
\footnotesize
\centering
\begin{tabular}{ |p{\dimexpr\linewidth-4\tabcolsep-1.5pt}| }
\toprule

\multicolumn{1}{|p{\dimexpr\linewidth-4\tabcolsep-1.5pt}|}{
{\textbf{Problem}: An $\textit{emirp}$ is an integer that, when its digits are written in reverse order, is a prime number. For example, 73 is an emirp because 37 is prime. What is the smallest two-digit prime number that is NOT an emirp?}
} \\
\midrule
{\textbf{Solution}: 

Step1: To determine the smallest two-digit prime number that is not an emirp, we need to follow these steps: First,\ \ldots\ldots\newline \ldots \newline
Step7: Continue to the next smallest two-digit prime number. 19 is prime.\newline
{\color{red}Step 8: Check if 23 is an emirp. Reverse the digits of 23: \(32\). Check if 32 is prime: No, 32 is not prime (divisible by 2). Since 23 is a prime number and its reverse, 32, is not a prime number, 23 is not an emirp. Therefore, the smallest two-digit prime number that is not an emirp is \(\boxed{23}\).}
} \\
\midrule
{\textbf{Qwen2.5-Math-7B-PRM800K} score: {\color{red}0.86}}
\\
\midrule
{\textbf{Qwen2.5-Math-PRM-7B} score: {\color{red}0.99}}
\\
\midrule
{\textbf{R-PRM}: Analysis: Previous Steps Analysis: 1. Step 1: This step starts by identifying the smallest two-digit prime numbers, \ \ldots\newline
Now Step Analysis: The Now Step checks if 23 is an emirp. It reverses the digits of 23 to get 32 and checks if 32 is prime.\ \ldots\ldots
\newline\ %\ldots\ldots\newline
Calculation Analysis: The calculation in the Now Step involves checking if 32 is prime. Since 32 is indeed divisible by 2 (32 = 2 * 16), \ \ldots\ldots The actual check for the smallest should consider all numbers in sequence. \textbf{\color{blue}Upon reviewing, the mistake in the analysis is assuming 23 is the answer without properly checking if there are smaller primes that are not emirps}. The sequence provided missed checking the next few primes after 17 (19, 23) more thoroughly. Since 19 is also a prime and its reverse is 91, which is not prime (91 = 7 * 13), 19 is actually not an emirp. Thus, the correct smallest two-digit prime that is not an emirp, based on the definition provided, should indeed consider all primes in ascending order. \textbf{\color{blue}Given the oversight in the analysis regarding the thorough checking of primes and their reversals, the conclusion that 23 is the smallest such prime without properly validating against all primes in sequence is premature.} \ \ldots\ldots\newline
Conclusion: \textbf{\color{blue}The Now Step incorrectly concludes that 23 is the smallest two-digit prime number that is not an emirp without properly validating against all primes in sequence and their reversals.} \ \ldots\ldots\newline
Verification: Is the step correct (Yes/No)? No
} \\
\midrule
{\textbf{R-PRM} score: {\color{blue}0.05}}
\\
\bottomrule
\end{tabular}
\caption{
 A case study from MATH subset of ProcessBench. {\color{red}Red} text denotes the error step and the scores of other models, and the {\color{blue}blue} text highlights our model's critique of the error and our score for that step.
}
\vspace{-0.3cm}
\label{case-study-2}
\end{figure*}

==> latex/tables/data_source.tex <==
% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Model} & \textbf{Data Source} & \textbf{Data Scale} \\
% \hline
% Math-Shepherd & MetaMath & 445k \\
% \hline
% MATH-PSA & Math-Shepherd + PRM500K + MATH-PAS & 1,097k \\
% \hline
% RLHFlow-DeepSeek & MetaMath & 253k \\
% \hline
% RLHFlow-Mistral & MetaMath & 273k \\
% \hline
% Qwen-2.5-Math-PRM & - & 1.8M \\
% \hline
% Llemma-PRM800K & MATH, PRM800K & 130k \\
% \hline
% Llemma-MetaMath & MATH, MetaMath & 108k \\
% \hline
% ReasonEval & PRM800K & 75k \\
% \hline
% Qwen2.5-Math-7B-PRM800K & PRM800K & 265k \\
% \hline

% \end{tabular}
% \caption{Data Models and Sources}
% \end{table*}

